Bi-directional Domain Adaptation for Sim2Real Transfer of Embodied Navigation Agents

Deep reinforcement learning models are notoriously data hungry, yet real-world data is expensive and time consuming to obtain. The solution that many have turned to is to use simulation for training before deploying the robot in a real environment. Simulation offers the ability to train large numbers of robots in parallel, and offers an abundance of data. However, no simulation is perfect, and robots trained solely in simulation fail to generalize to the real-world, resulting in a "sim-vs-real gap". How can we overcome the trade-off between the abundance of less accurate, artificial data from simulators and the scarcity of reliable, real-world data? In this paper, we propose Bi-directional Domain Adaptation (BDA), a novel approach to bridge the sim-vs-real gap in both directions -- real2sim to bridge the visual domain gap, and sim2real to bridge the dynamics domain gap. We demonstrate the benefits of BDA on the task of PointGoal Navigation. BDA with only 5k real-world (state, action, next-state) samples matches the performance of a policy fine-tuned with ~600k samples, resulting in a speed-up of ~120x.

==> sections/4_system_architecture.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{System Architecture}
\label{sec:sys_arch}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \label{sec:domain_adapt}
% \IncMargin{1em}
% \begin{algorithm}
% \SetAlgoNoLine%
% \small 
% \sourcenn $\leftarrow$ Initial source simulation with no noise\\
% Train behavior policy \pisource in \sourcenn\\
% \For{$t$ = 0, ..., N \text{steps}}{
%  Collect \imgtnn $\sim$  \targetnn rollout (\pisource)\\
%  Collect \imgtn, \stn, \atn $\sim$  \targetn rollout (\pisource) \\
% }
% Train \oa(\imgnn, \imgn)\\
% Train \da(\sn, \an)\\
% \sourceDA $\leftarrow$ Augment Source with \da \\
% \For{$j$ = 0, ..., K \text{steps}}{
%  \piDA $\leftarrow$ Finetune \pisource in \sourceDA
% }
% \piODA $\leftarrow$ Apply \oa at test-time\\
% Test \piODA in \targetn 
%  \caption{Bi-directional Domain Adaptation}
%  \label{alg:architecture}
% \end{algorithm}
% \DecMargin{1em}

% In this section, we describe how we instantiate \refalg{alg:architecture} in the context of PointNav. We begin by training a behavior policy, \pis (line 2). We sample 5,000 rollouts of \pis in \labnn and \labn to collect at time $t$, RGB-D images \imgtnn and \imgtn, as well as state-action pairs along the robot's trajectory (\stn, \atn), with \stn = ($x^{O+D}_t$, $y^{O+D}_t$, cos$\theta^{O+D}_t$, sin$\theta^{O+D}_t$) (lines 3-5). 

% The dataset of unpaired images from the source and target environments \imgnnd and \imgnd are used to train a observation adaptation module, \oa, which learns to translate \imgnd $\mapsto$ \imgnnd (line 6). 
% We train \oa from scratch for 200 epochs. From \reffig{fig:cyc}, we see that the model learns to remove the Gaussian noise placed on the RGB image, and learns to smooth out textures in the depth image. 

% The state (\sn)  and action (\an)  pairs are used to train a dynamics adaptation module, \da, which learns to predict the robot's position and orientation after taking an action, if the action were to have taken place in the real-world (line 7). Specifically, we concatenate \sn with a one hot encoding of the action \an as input to a 3 layer multilayer perceptron regression network. The neural network learns to estimate the change in position and orientation $\Delta s^{O+D}$ ($s^{O+D}_{t+1} - s^{O+D}_t)$. We use a weighted MSE loss function,  $\frac{1}{n}\sum_{n=1}^{N}\mathbf{w}^\top(\Delta s^{O+D}_{n}- \Delta \hat{s}^{O+D}_{n})^2$. Given the cylindrical morphology of the robot, we placed weighed the prediction terms for the robot's position twice as high as the weights for its angle because getting the position correct is more important for ensuring that a higher SPL is achieved.  

% Once trained, \da is used to augment the source environment (line 8). We finetune \pis in the augmented source environment, \sourceDA (lines 9-10). We use \oa at test time (line 11). Finally, we test our policy trained with BDA in \targetn (line 12). BDA allows us to learn a policy that is able to adapt to the noise present in \labn, while avoiding overfitting to the new data.

% \xhdr{Observation Adaptation.} To overcome the visual domain shift, we propose to train a \emph{real2sim} observation adaptation module \oa by using CycleGAN \cite{CycleGAN2017}, a pixel-level image-to-image translation technique. 
% % , at test time to translate RGB-D images from \labn ($\mathcal{T}$) to RGB-D images in \labnn ($\mathcal{S}$). 
% We collect RGB-D images from \labnn and \labn, and learn a mapping $\mathcal{G}_{sim}: \calI^{\text{real}} \mapsto \calI^{\text{sim}}$. Learning the mapping $\mathcal{G}_{sim}$ enables us to disentangle the sensor adaptation network from our policy training, so that if \labn changes, the base policy can be kept frozen, and only \oa will have to be retrained. In addition, CycleGAN uses unpaired images from both domains, which is important because it is difficult to accurately collect paired images in the real-world. 

% \xhdr{Dynamics Adaptation.} In addition to closing the visual domain gap, we attempt to close the dynamics gap by modeling the actuation noise on the mobile robot. Using rollouts in the target domain, we collect at time $t$, the robot's current state, $s_{t}$ ($x_t$, $y_t$, cos$\theta_t$, sin$\theta_t$), and action $a_t$ along the robot's trajectory. We train a 3 layer multilayer perceptron regression network to estimate the change in position and orientation $\Delta s$ ($s_{t+1} - s_t)$. As input, we concatenate $s_{t}$ with a one hot encoding of the action $a_t$. We use a weighted MSE loss function,  $\frac{1}{n}\sum_{n=1}^{N}w(\Delta s_{n}- \Delta \hat{s_{n}})^2$, with higher weights on prediction terms for the robot's position. 

